The computational asymptotics of Gaussian variational inference and the Laplace approximation

Gaussian variational inference and the Laplace approximation are popular alternatives to Markov chain Monte Carlo that formulate Bayesian posterior inference as an optimization problem, enabling the use of simple and scalable stochastic optimization algorithms. However, a key limitation of both methods is that the solution to the optimization problem is typically not tractable to compute; even in simple settings the problem is nonconvex. Thus, recently developed statistical guarantees -- which all involve the (data) asymptotic properties of the global optimum -- are not reliably obtained in practice. In this work, we provide two major contributions: a theoretical analysis of the asymptotic convexity properties of variational inference with a Gaussian family and the maximum a posteriori (MAP) problem required by the Laplace approximation; and two algorithms -- consistent Laplace approximation (CLA) and consistent stochastic variational inference (CSVI) -- that exploit these properties to find the optimal approximation in the asymptotic regime. Both CLA and CSVI involve a tractable initialization procedure that finds the local basin of the optimum, and CSVI further includes a scaled gradient descent algorithm that provably stays locally confined to that basin. Experiments on nonconvex synthetic and real-data examples show that compared with standard variational and Laplace approximations, both CSVI and CLA improve the likelihood of obtaining the global optimum of their respective optimization problems.

==> smoothedmap.tex <==
\subsection{Initialization via smoothed MAP}\label{sec:smoothedmap} 

The goal of this section is to design an algorithm that initializes 
the Laplace approximation and the variational optimization within the asymptotically strongly convex local
region $B_r$, $\mcB_{r,n}$ respectively. 
Note that initial covariance of the Gaussian variational inference can be
simply set as identity matrix. For mean intialization, 
we aim to set $\mu$ sufficiently close to $\mu_n^\star$---and $\mu_n^\star$ converges to
$\theta_0$ per \cref{thm:optimum_inside}---we might like to find something
akin to the maximum a posteriori (MAP) value of $\log \pi_n$, due to its
similar convergence to $\theta_0$, which can be also used for Laplace initialization. 



In this section, we formulate a tractable MAP-like problem by convolving the
posterior distribution with Gaussian noise prior to finding the maximum point
of the log density. This Gaussian noise essentially results in smoothed log
density with fewer spurious optima; hence, we denote this the \emph{smoothed
MAP problem}. In \cref{sec:smoothedpost}, we show that the smoothed MAP
problem is asymptotically convex---and hence tractable---under conditions
similar to those that guarantee the Bernstein-von Mises theorem, and that the
solution is asymptotically consistent for $\theta_0$, albeit at a
slower-than-$\sqrt{n}$ rate. In \cref{sec:smoothedmapopt}, we provide a
stochastic optimization algorithm that depends only on black-box access to
the gradients of the original log density function. Taken together, these
results demonstrate that we can tractably initialize CSVI in the
asymptotically strongly convex local region $\mcB_{r,n}$ as required.

\subsubsection{Smoothed MAP problem} \label{sec:smoothedpost}

Given the $n^\text{th}$ posterior distribution $\Pi_n$, we define the \emph{smoothed posterior} $\hPi_n$
with smoothing variance $\alpha_n$ to be the $\theta$-marginal of the  generative process
\[
W \dist \Pi_n, \quad \theta \dist \distNorm(W, \alpha_n I).	
\]
Alternatively, the smoothed posterior distribution $\hPi_n$ can be viewed as
the distribution of the sum of independent
realizations from $\Pi_n$ and $\distNorm(0, \alpha_n I)$.
The probability density function $\hpi_n$ of $\hPi_n$ is given by the
convolution
of $\pi_n$ with a multivariate normal density,
\[ 
\hat{\pi}_n(\theta) =&  \int \frac{1}{(2\pi)^{d/2} \alpha_n^{d/2}} \exp\left( -\frac{1}{2\alpha_n}\|\theta - w \|^2 \right) \pi_n(w) dw \\
=& \EE\left[\frac{1}{(2\pi)^{d/2} \alpha_n^{d/2}} \exp\left( -\frac{1}{2\alpha_n}\|\theta - W \|^2 \right)\right]. \label{eq:smootheddensity}
\]
Given these definitions, the \emph{smoothed MAP problem} is the MAP inference problem for the smoothed posterior distribution, i.e.,
\[ \label{eq:smoothedmap}
\hat{\theta}_{n} =&
\argmin_{\theta \in \reals^d } \,\, - \log \EE\left[\exp\left(-\frac{1}{2\alpha_n}\| \theta - W\|^2\right)\right].
\]

Gaussian smoothing is commonly used in image and signal processing
\citep{forsyth2002computer,nixon2012feature,haddad1991class,lindeberg1990scale},
and has previously been applied to reduce the presence of spurious local
optima in nonconvex optimization problems, making them easier to solve with
local gradient-based methods \citep{addis2005local,mobahi2013optimization}.
The variance $\alpha_n$ controls the degree of smoothing; larger values
create a smoother density $\hpi_n$, at the cost of making $\hpi_n$ a poorer
approximation of the original function $\pi_n$. \cref{fig:smoothing}
demonstrates how increasing $\alpha_n$ increases the smoothing effect,
resulting in fewer and flatter local optima in the objective.

\begin{figure}[t!]
	\centering
	\includegraphics[width = \linewidth]{figures/toy_smooth_posts.png}
	\caption{Plots of the smoothed posterior density $\hpi_n$ with increasing smoothing variance $\alpha$. Note that $\alpha = 0$ denotes the original posterior.}
	\label{fig:smoothing}
\end{figure}

In general, although intuitively reasonable, the Gaussian smoothing method does not
typically come with strong practical theoretical guarantees, essentially
because the best choice of the smoothing variance $\alpha_n$ is not known.
\citet{mobahi2013optimization} shows for a continuous integrable function
with quickly decaying tails (at rate $\|x\|^{-d-3}$ as $\|x\|\to\infty$), the
smoothed function is strictly convex given a large enough selection of
$\alpha_n$. \citet{addis2005local} studies the smoothing effect of a
log-concave kernel on a special type of piecewise constant function, and
proves that the smoothed function is either monotonic or unimodal. To the
best of our knowledge, previous analyses of smoothed optimization are not
sufficient to guide the choice of $\alpha_n$ and do not provide bounds on the
error of the smoothed optimum point versus the original.

In contrast to these previous studies, we use the asymptotic concentration of the
statistical model as $n\to\infty$ to address both of these
issues. In particular, \cref{thm:convexsmoothedMAP} shows that if the sequence
$\alpha_n$ is chosen to decrease more slowly than $n^{-1/3}$, the smoothed MAP
problem is eventually strictly convex within any arbitrary compact domain;
and that the solution of the smoothed MAP problem is asymptotically
consistent for $\theta_0$ at a $\sqrt{\alpha_n}^{-1}$ rate. 
\bnthm \label{thm:convexsmoothedMAP}
Suppose \cref{assump:regularity} holds and $n \alpha_n^3 \to
\infty$. Then for all $M>0$, the probability that the smoothed MAP optimization problem 
\[
\min_{\|\theta-\theta_0\|\leq M}  - \log \hat{\pi}_n(\theta)
\]
is strictly convex converges to $1$ as $n \to \infty$ under the data generating
distribution. Further, the optima for the smoothed MAP problem is asymptotically $\sqrt{\alpha_n}$-consistent, that is
\[
	\|\hat{\theta}_{n} - \theta_{0}\| = O_{P_{\theta_0}}(\sqrt{\alpha_n}).
\]
\enthm




\subsubsection{Smoothed MAP optimization}\label{sec:smoothedmapopt}

In practice, we use SGD to solve the smoothed MAP problem. The 
gradient of the smoothed MAP objective function in \cref{eq:smoothedmap} is
\[
& \nabla (-\log \hat{\pi}_n(\theta)) \\
& = -\nabla \log \EE\left[\exp\left(-\frac{1}{2\alpha_n}\| \theta - W\|^2\right)\right] \\
& = -\frac{ \EE\left[\exp\left(-\frac{1}{2\alpha_n}\| \theta - W\|^2\right) \left(- \frac{1}{\alpha_n} \right) \left( \theta-W \right)\right]}{\EE\left[\exp\left(-\frac{1}{2\alpha_n}\| \theta - W\|^2\right)\right]},
\]
where $W \sim \Pi_n$. By change of variables and reparametrization,
the gradient can be reformulated as
\[\label{eq:smoothgrd}
\nabla (-\log \hat{\pi}_n(\theta) )
%=& \frac{\left(-\frac{1}{\alpha_n}\right) \EE_u\left[u p_n(\theta-u)\right]}{\EE_u\left[p_n(\theta-u)\right]}\\
=&\, \alpha_n^{-1/2} \frac{
\EE\left[W \pi_n\left(\theta-\alpha_n^{1/2} W\right)\right]
}{
\EE\left[\pi_n\left(\theta- \alpha_n^{1/2}W\right)\right]
},
\]
where $W \sim \distNorm\left(0, I\right)$. Note that the unknown
normalization constant in $\pi_n$ cancels in the numerator and denominator.
We obtain stochastic estimates of the gradient using a Monte Carlo
approximation of the numerator and denominator using the same samples, i.e.,
self-normalized importance sampling \citep[p.~95]{robert2013monte}. It is
known that the variance of this gradient estimate may be quite large or even
infinite; although techniques such as truncation \citep{ionides2008truncated}
and smoothing \citep{vehtari2015pareto} exist to address it, we leave this
issue as an open problem for future work. The resulting SGD procedure with
explicit gradient estimates are shown in \cref{alg:smoothedmap}. 
 
To visualize the behaviour of the smoothed MAP optimization, we construct a
synthetic Bayesian model where the posterior distribution, displayed in
\cref{fig:posts}, is asymptotically normal but has multiple modes even given
a large sample size. The details of this synthetic model and the setting of
the experiment can be found in \cref{supp:smoothexample}. The spurious local
optima make local optimization methods unreliable. In contrast,
\cref{fig:smthedmaps} shows that the smoothed posterior has fewer modes and
is able to maintain the asymptotic normality of the true posterior, which
aligns with the analysis in \cref{thm:convexsmoothedMAP}. Thus, the smoothed
posterior can be used to find a reliable initialization for Gaussian
variational inference.

 

   

\begin{algorithm}[t!]
\caption{Smoothed MAP estimation} \label{alg:smoothedmap}
\begin{algorithmic}
\Procedure{SmoothedMAP}{$\pi_n$, $\alpha_n$, $x_0$, $K$, $S$, $(\gamma_k)_{k\in\nats}$}
\For{$k=0, 1, \dots, K-1$}
	\State Sample $(Z_s)_{s = 1}^S \distiid \distNorm(0,I)$
	\State $\hat\nabla_k \!\gets \alpha_n^{-\frac{1}{2}}\!\left(\!\sum_{s = 1}^S \!Z_s \! \pi_n(x_k-\alpha_n^{\frac{1}{2}}Z_s)\!\right)\!\Big/\!\left(\!\sum_{s = 1}^S\pi_n(x_k- \alpha_n^{\frac{1}{2}}Z_s)\!\right) $ 
	\State $x_{k+1} \gets x_k - \gamma_k \hat\nabla_k$ 
\EndFor
\State \Return $x_K$
\EndProcedure
\end{algorithmic}
\end{algorithm}

